NaRA: Noise-Aware LoRA for Parameter-Efficient Fine-Tuning of Diffusion LLMs

Diffusion Large Language Models (dLLMs) have emerged as a promising non-autoregressive generative paradigm. Given the prohibitive computational cost of full fine-tuning, Parameter-Efficient Fine-Tuning (PEFT) has become the standard approach. However, existing PEFT methods (e.g., LoRA), originally tailored for autoregressive models, rely on static parameters that are agnostic to the noise level. Consequently, they ignore the intrinsic dynamics of the diffusion process, where input distributions and generation difficulty shift significantly along the denoising trajectory, rendering them suboptimal for dLLMs. To address this, we propose Noise-aware Low-Rank Adaptation (NaRA), which introduces a low-rank core matrix generated by a lightweight, globally shared hypernetwork conditioned on the noise level. This design enables the update matrices to vary continuously along the diffusion process while keeping parameter and latency overhead negligible. We provide a theoretical justification for the proposed NaRA framework and empirically demonstrate consistent improvements over noise-agnostic baselines across commonsense reasoning, mathematical reasoning, and code generation benchmarks. Our code is available at https://github.com/generaldi/NaRA.

==> tabs/app_efficiency.tex <==
\begin{table}[h]
\centering
\caption{Comparison of training and inference time. We measure total training and inference GPU hours.}
\label{tab:efficiency_appendix}
\begin{small}
\begin{sc}
\begin{tabular}{llcc}
\toprule
Dataset & Method & Training & Inference \\ % 合并并增加了单位
\midrule
\multirow{2}{*}{Commonsense} 
& LoRA & 18.82 & 7.78 \\
& NaRA & 18.62 & 7.47 \\
\midrule
\multirow{2}{*}{Math} 
& LoRA & 14.53 & 12.09 \\
& NaRA & 14.07 & 11.95 \\
\midrule
\multirow{2}{*}{Code} 
& LoRA & 5.43 & 7.99 \\
& NaRA & 4.87 & 8.46 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{table}

==> tabs/app_per_step_infer.tex <==
\begin{table}[h]
\centering
\caption{Per-step inference time and peak VRAM.}
\vspace{-5pt}
\label{tab:per_step_infer}
\begin{small}
\begin{sc}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l l cc}
\toprule
Length & Method & Step Time (ms) & Peak VRAM (GB) \\
\midrule
\multirow{3}{*}{256}
 & LoRA (merged)   & 88.10  & 16.11 \\
 & LoRA (unmerged) & 92.88  & 16.18 \\
 & NaRA (Ours)     & 92.57  & 16.18 \\
\midrule
\multirow{3}{*}{1024}
 & LoRA (merged)   & 331.34 & 16.31 \\
 & LoRA (unmerged) & 344.74 & 16.38 \\
 & NaRA (Ours)     & 344.96 & 16.38 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{table}

==> tabs/app_per_step_train.tex <==
\begin{table}[h]
\centering
\caption{Per-step training time and peak VRAM after implementation normalization.}
\vspace{-5pt}
\label{tab:per_step_train}
\begin{small}
\begin{sc}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l l cc}
\toprule
Length & Method & Step Time (ms) & Peak VRAM (GB) \\
\midrule
\multirow{3}{*}{256}
 & LoRA (original) & 261.68 & 18.21 \\
 & LoRA (fixed)    & 248.89 & 18.21 \\
 & NaRA (Ours)     & 254.55 & 18.22 \\
\midrule
\multirow{3}{*}{1024}
 & LoRA (original) & 791.57 & 23.28 \\
 & LoRA (fixed)    & 768.48 & 23.28 \\
 & NaRA (Ours)     & 770.23 & 23.30 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{table}
